OneEdit: A Neural-Symbolic Collaboratively Knowledge Editing System

Knowledge representation has been a central aim of AI since its inception. Symbolic Knowledge Graphs (KGs) and neural Large Language Models (LLMs) can both represent knowledge. KGs provide highly accurate and explicit knowledge representation, but face scalability issue; while LLMs offer expansive coverage of knowledge, but incur significant training costs and struggle with precise and reliable knowledge manipulation. To this end, we introduce OneEdit, a neural-symbolic prototype system for collaborative knowledge editing using natural language, which facilitates easy-to-use knowledge management with KG and LLM. OneEdit consists of three modules: 1) The Interpreter serves for user interaction with natural language; 2) The Controller manages editing requests from various users, leveraging the KG with rollbacks to handle knowledge conflicts and prevent toxic knowledge attacks; 3) The Editor utilizes the knowledge from the Controller to edit KG and LLM. We conduct experiments on two new datasets with KGs which demonstrate that OneEdit can achieve superior performance.

==> CASE/table1.tex <==
\begin{table*}[ht!]
\centering
\caption{Comparison of OneEdit to existing methods. Metrics shown are computed after all single edits. In OneEdit, we set the number of generation triples to 8}
\label{tab1}
\setlength{\extrarowheight}{0.5pt} 
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
& \multicolumn{6}{c|}{\textbf{American politicians dataset}}&\multicolumn{6}{c}{\textbf{Academic Figures dataset}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13} 
\multirow{2}{*}{Method} & \multirow{2}{*}{Reliability} & \multirow{2}{*}{Locality} & \multicolumn{3}{c}{Portability} & \multirow{2}{*}{Average}&  \multirow{2}{*}{Reliability} & \multirow{2}{*}{Locality} & \multicolumn{3}{c}{Portability} & \multirow{2}{*}{Average} \\
\cmidrule(lr){4-6} \cmidrule(lr){10-12}
 & & & Reverse & One-Hop & Sub-Replace & & & & Reverse & One-Hop & Sub-Replace \\
\midrule
% \scriptsize \textbf{GPT2-XL} \\
% \midrule
% FT          & 0.728     & 0.451     & 0.239     & 0.167     & 0.293     & 0.376 
%             & 0.603     & 0.456     & 0.167     & 0.191     & 0.287     & 0.341\\
% ROME        & 0.999     & 0.998     & 0.506     & 0.309     & 0.796     & 0.722 
%             & 0.998     & 0.962     & 0.686     & 0.314     & 0.864     & 0.765 \\
% MEMIT       & 0.982     & 0.997     & 0.570     & 0.401     & 0.568     & 0.704 
%             & 0.970     & 0.979     & 0.612     & 0.351     & 0.769     & 0.736 \\
% GRACE       & \textbf{1.000}     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.400 
%             & \textbf{1.000}     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.400 \\
% \midrule
% OneEdit (GRACE)      & 0.952     & \textbf{1.000}     & \textbf{0.973}     & \textbf{0.950}     & \textbf{0.968}&   \textbf{0.967} 
%                     & 0.967     & \textbf{1.000}     & \textbf{0.979}     & \textbf{0.962}     & \textbf{0.968}& \textbf{0.894}\\
% OneEdit (MEMIT)      & 0.831     & 0.933     & 0.853     & 0.609     & 0.842    & 0.809  
%                     & 0.869     & 0.953     & 0.948     & 0.695    & 0.908    & 0.875\\
% \midrule
\scriptsize \textbf{GPT-J-6B} \\
\midrule
FT          & 0.825     & 0.008     & 0.240     & 0.034     & 0.620     & 0.339 
            & 0.571     & 0.008     & 0.610     & 0.000     & 0.620     & 0.362\\
ROME        & 0.996     & 0.982     & 0.235     & 0.176     & 0.828     & 0.634 
            & 0.994     & 0.982     & 0.561     & 0.175     & 0.906     & 0.724 \\
MEMIT       & \textbf{1.000}        & 0.997     & 0.581     & 0.402     & 0.554     & 0.736 
            & 0.996     & 0.997     & 0.665     & 0.055     & 0.799     & 0.702\\
GRACE       & \textbf{1.000}     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.400 
            & \textbf{1.000}     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.400\\
\midrule
OneEdit (GRACE)      & 0.951     & \textbf{1.000}     & 0.950     & \textbf{0.928}     & 0.922    & 0.950 & 0.952     
                    & \textbf{1.000}     & \textbf{0.991}     & \textbf{0.958}     & \textbf{0.962}    & \textbf{0.973}\\
OneEdit (MEMIT)      & \textbf{0.995}     & 0.947     & \textbf{0.957}     & 0.713     & \textbf{0.952}    & value
                    & \textbf{0.982}     & 0.933     & 0.987     & 0.722     & 0.842    & 0.865\\

\bottomrule


\scriptsize \textbf{Qwen2-7B} \\
\midrule
FT          & 0.662     & 0.012     & 0.512     & 0.237     & 0.660     & value 
            & 0.601     & 0.103     & 0.610     & 0.139     & 0.633     & value\\
ROME        & 0.996     & 0.982     & 0.623     & 0.399     & 0.727     & 0.634 
            & 0.994     & 0.982     & 0.528     & 0.417     & 0.774     & 0.724 \\
MEMIT       & 0.972     & 0.986     & 0.665     & 0.402     & 0.652     & 0.736 
            & 0.996     & 0.993     & 0.665     & 0.422     & 0.698     & 0.702\\
GRACE       & \textbf{1.000}     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.400 
            & \textbf{1.000}     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.400\\

\midrule
OneEdit (GRACE)      & 0.953     & \textbf{1.000}     & 0.962     & 0.958     & 0.943    &value 
                     & 0.961     & \textbf{1.000}     & 0.958     & 0.951     & 0.949    &value\\
                     
OneEdit (MEMIT)      & \textbf{0.955}     & 0.956     & 0.923     & 0.763     & 0.966    & value 
                     & \textbf{0.973}     & 0.963     & 0.957     & 0.697     & 0.942    & value\\

\bottomrule


\end{tabular}   }
\end{table*}





%两个表，第一个表是single加reverse的，改成 rel loc por_gen por_rev por_mh
%第二个表是coverage不同n的指标，整个n=2，n=3就行了，测一下rel loc por_gen por_rev por_mh
%baseline 就是ft rome grace 和OneEdit

% \begin{table}[ht]
% \centering
% \caption{Detailed GPT2XL Metrics Across Different Methods}
% \label{tab1}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}lccccc@{}}
% \toprule
%  \multirow{2}{*}{Method}  &     &  & \multicolumn{3}{c}{Portability} \\
% \cmidrule(lr){4-6}
%        &Reliability  & Locality & Reverse & One-Hop & Sub-Replace\\
% \midrule
% \multicolumn{6}{c}{GPT2-XL} \\
% \midrule
% FT         & value       & value    & value   & value   & value     \\
% ROME       & 0.999       & 0.483    & 0.188   & 0.507   & value     \\
% GRACE      & 0.961       & 1.000    & 0.000   & 0.000   & value     \\
% OneEdit  & 0.952       & 1.000    & 0.973   & 0.950   & value     \\
% \usepackage{}
% \midrule
% \multicolumn{6}{c}{GPTJ-6B} \\
% \midrule
% FT         & value       & value    & value   & value   & value     \\
% ROME       & 0.999       & 0.483    & 0.188   & 0.507   & value     \\
% GRACE      & 0.961       & 1.000    & 0.000   & 0.000   & value     \\
% OneEdit  & 0.952       & 1.000    & 0.973   & 0.950   & value     \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

==> CASE/table2.tex <==
\begin{table*}[ht!]
\centering
\caption{Comparison of OneEdit to existing methods in a multi-user scenario. User=2 indicates that a single piece of knowledge has been edited twice, once by each of two users. Similarly, when the number of users is 3, the knowledge has been edited three times, once by each user.}
\label{tab2}
\setlength{\extrarowheight}{-2pt} 
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Reliability} & \multirow{2}{*}{Locality} & \multicolumn{3}{c}{Portability} & \multirow{2}{*}{Average} \\
\cmidrule(lr){4-6}
 & & & Reverse & One-Hop & Sub-Replace & \\
\midrule
\scriptsize \textbf{GPT2-XL, Users = 2} \\
\midrule
FT          & 0.691     & 0.275     & 0.168     & 0.114     & 0.121     & 0.274 \\
ROME        & 0.981     & 0.641     & 0.392     & 0.283     & 0.706     & 0.601 \\
MEMIT       & 0.972     & 0.998     & 0.560     & 0.412     & 0.503     & 0.689 \\
GRACE       & \textbf{1.000}     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.400 \\
\midrule
OneEdit (GRACE)      & 0.952     & \textbf{1.000}     & \textbf{0.892}     & 0.729     & \textbf{0.918}     & \textbf{0.898} \\
OneEdit (MEMIT)       & 0.851     & 0.993     & 0.862    & \textbf{0.871}     & 0.859     & 0.866 \\
\midrule
\scriptsize \textbf{GPT-J-6B, Users = 2} \\
\midrule
FT          & 0.902     & 0.082     & 0.249     & 0.000     & 0.590     & 0.365 \\
ROME        & 0.987     & 0.040     & 0.156     & 0.067     & 0.629     & 0.376 \\
MEMIT       & 0.998     & 0.421     & 0.156     & 0.399     & 0.526     & 0.500 \\
GRACE       & \textbf{1.000}     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.400 \\
\midrule
OneEdit (GRACE)       & 0.952     & \textbf{1.000}     & 0.802     & 0.730     & 0.824     & 0.862 \\
OneEdit (MEMIT)       & 0.833     & 0.989     & \textbf{0.849}     & 0.706     & \textbf{0.842}    & 0.844 \\
\midrule
\scriptsize \textbf{GPT2-XL, Users = 3} \\
\midrule
FT          & 0.797     & 0.210     & 0.165     & 0.102     & 0.120     & 0.279 \\
ROME        & \textbf{0.999}     & 0.483     & 0.266     & 0.215     & 0.701     & 0.533 \\
MEMIT       & \textbf{0.999}     & 0.998     & 0.544     & 0.380     & 0.593     & 0.703 \\
GRACE       & 0.961     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.392 \\
\midrule
OneEdit (GRACE)       & 0.952     & \textbf{1.000}     & 0.892     & 0.850     & \textbf{0.918}     & \textbf{0.922} \\
OneEdit (MEMIT)       & 0.853     & 0.994     & \textbf{0.859}    & \textbf{0.866}     & 0.862     & 0.863 \\
\midrule
\scriptsize \textbf{GPT-J-6B, Users = 3} \\
\midrule
FT          & 0.850     & 0.059     & 0.210     & 0.000     & 0.588     & 0.341 \\
ROME        & 0.988     & 0.006     & 0.122     & 0.003     & 0.608     & 0.345 \\
MEMIT       & 0.987     & 0.328     & 0.544     & 0.380     & 0.523     & 0.552 \\
GRACE       & \textbf{0.999}     & \textbf{1.000}     & 0.000     & 0.000     & 0.000     & 0.399 \\
\midrule
OneEdit (GRACE)       & 0.952     & \textbf{1.000}     & 0.802     & \textbf{0.850}     & 0.824     & \textbf{0.886} \\
OneEdit (MEMIT)       & 0.832     & 0.983     & \textbf{0.856}     & 0.749     & \textbf{0.852}    & 0.854 \\
\bottomrule
\end{tabular}
}
\end{table*}

% \begin{table}[ht]
% \centering
% \caption{Detailed GPT2XL Metrics Across Different Methods}
% \label{tab2}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}l ccc ccc@{}}
% \toprule
%             & \multicolumn{3}{c}{Coverge n=2}    & \multicolumn{3}{c}{Coverge n=3} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% Method      & Relibility   & Locality   & Portability-avg   & Relibility   & Locality   & Portability-avg\\
% \midrule
% FT          & value & value & value & value & value & value     \\
% ROME        & 0.999 & 0.823 & value & value & value & value     \\
% GRACE       & 0.961 & 1.000 & value & value & value & value     \\
% OneEdit   & 0.952 & 1.000 & value & value & value & value     \\
% \midrule
% \end{tabular}
% }
% \end{table}
%两个表，第一个表是single加reverse的，改成 rel loc por_gen por_rev por_mh
%第二个表是coverage不同n的指标，整个n=2，n=3就行了，测一下rel loc por_gen por_rev por_mh
%baseline 就是ft rome grace 和OneEdit

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
